A Most Interesting, but Revoked Draft for Hilbert and Bernays' "Grundlagen der Mathematik" that never found its way into any publication, and 2 CV of Gisbert Hasenjaeger

In 1934, in Bernays preface to the 1st edn. of the 1st vol. of Hilbert-Bernays "Grundlagen der Mathematik", a nearly completed draft of the the finally two-volume monograph is mentioned, which had to be revoked because of the completely changed situation in the area of proof theory after Herbrand and Goedels revolutionary results. Nothing at all seems to be known about this draft and its whereabouts. A third of a century later, Bernays preface to the 2nd edn. (1968) of the 1st vol. of Hilbert-Bernays mentions joint work of Hasenjaeger and Bernays on the second edition. Bernays states there that it became obvious that the integration of the many new results in the area of proof theory would have required a complete reorganization of the book, i.e. that the inclusion of the intermediately found new results in the area of proof theory turned out to be unobtainable by a revision, but would have required a complete reorganization of the entire textbook. We document that - even after the need for a complete reorganization had become obvious - this joint work went on to a considerable extent. Moreover, we document when Hasenjaeger stayed in Zurich to assist Bernays in the completion of the 2nd edn. In May 2017, we identified an incorrectly filed text in Bernays scientific legacy at the archive of the ETH Zurich as a candidate for the beginning of the revoked draft for the 1st edn. or of a revoked draft for the 2nd edn. In a partial presentation and careful investigation of this text we gather only some minor evidence that this text is the beginning of the nearly completed draft of the 1st edn., but ample evidence that this text is part of the work of Hasenjaeger and Bernays on the 2nd edn. We provide some evidence that this work has covered a complete reorganization of the entire 1st vol., including a completely new version of its last chapter on the iota.

==> headerhot.tex <==
\def\subsubsubsection{\paragraph}
\def\subsubsubsubsection{\subparagraph}
\catcode`\@=11
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\font\sixsf  = cmss10 scaled 600
\font\fvesf  = cmss10 scaled 500
%\font\sevsf  = cmss10 scaled 700
\font\egtsf  = cmss10 scaled 800
%\font\twfvit  = cmti10   \@magscale5 % text italic

\def\xiipt{\textfont\z@\twlrm 
  \scriptfont\z@\egtrm \scriptscriptfont\z@\sixrm
\textfont\@ne\twlmi \scriptfont\@ne\egtmi \scriptscriptfont\@ne\sixmi
\textfont\tw@\twlsy \scriptfont\tw@\egtsy \scriptscriptfont\tw@\sixsy
\textfont\thr@@\tenex \scriptfont\thr@@\tenex \scriptscriptfont\thr@@\tenex
\def\unboldmath{\everymath{}\everydisplay{}\@nomath\unboldmath
          \textfont\@ne\twlmi 
          \textfont\tw@\twlsy \textfont\lyfam\twlly
          \@boldfalse}\@boldfalse
\def\boldmath{\@ifundefined{twlmib}{\global\font\twlmib\@mbi\@magscale1\global
        \font\twlsyb\@mbsy \@magscale1\global\font
         \twllyb\@lasyb\@magscale1\relax\@addfontinfo\@xiipt
              {\def\boldmath{\everymath
                {\mit}\everydisplay{\mit}\@prtct\@nomathbold
                \textfont\@ne\twlmib \textfont\tw@\twlsyb 
                \textfont\lyfam\twllyb\@prtct\@boldtrue}}}{}\@xiipt\boldmath}%
\def\prm{\fam\z@\twlrm}%
\def\pit{\fam\itfam\twlit}\textfont\itfam\twlit \scriptfont\itfam\egtit
   \scriptscriptfont\itfam\sevit
\def\psl{\fam\slfam\twlsl}\textfont\slfam\twlsl 
     \scriptfont\slfam\tensl \scriptscriptfont\slfam\tensl
\def\pbf{\fam\bffam\twlbf}\textfont\bffam\twlbf 
   \scriptfont\bffam\ninbf \scriptscriptfont\bffam\ninbf 
\def\ptt{\fam\ttfam\twltt}\textfont\ttfam\twltt
   \scriptfont\ttfam\nintt \scriptscriptfont\ttfam\nintt 
\def\psf{\fam\sffam\twlsf}\textfont\sffam\twlsf
    \scriptfont\sffam\egtsf \scriptscriptfont\sffam\sixsf
\def\psc{\@getfont\psc\scfam\@xiipt{\@mcsc\@magscale1}}%
\def\ly{\fam\lyfam\twlly}\textfont\lyfam\twlly 
   \scriptfont\lyfam\egtly \scriptscriptfont\lyfam\sixly
 \@setstrut \rm}

\def\xxvpt{\textfont\z@\twfvrm 
  \scriptfont\z@\twtyrm \scriptscriptfont\z@\svtnrm
\textfont\@ne\twtymi \scriptfont\@ne\twtymi \scriptscriptfont\@ne\svtnmi
\textfont\tw@\twtysy \scriptfont\tw@\twtysy \scriptscriptfont\tw@\svtnsy
\textfont\thr@@\tenex \scriptfont\thr@@\tenex \scriptscriptfont\thr@@\tenex
\def\unboldmath{\everymath{}\everydisplay{}\@nomath\unboldmath
        \textfont\@ne\twtymi \textfont\tw@\twtysy \textfont\lyfam\twtyly
        \@boldfalse}\@boldfalse
\def\boldmath{\@subfont\boldmath\unboldmath}%
\def\prm{\fam\z@\twfvrm}%
\def\pit{\fam\z@\twfvit}%
\def\psl{\@subfont\sl\rm}%
\def\pbf{\@getfont\pbf\bffam\@xxvpt{cmbx10\@magscale5}}%
\def\ptt{\@subfont\tt\rm}%
\def\psf{\@subfont\sf\rm}%
\def\psc{\@subfont\sc\rm}%
\def\ly{\fam\lyfam\twtyly}\textfont\lyfam\twtyly 
   \scriptfont\lyfam\twtyly \scriptscriptfont\lyfam\svtnly 
\@setstrut \rm}

\catcode`\@=12


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SUPERCOMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The following redefines the latex macro \math not because 
% \math makes trouble but rather because I dont like it
\long\def\math#1{\relax\ifmmode{#1}\else$#1 $\fi}
%                                          ^ 
% This blank is necessary because otherwise \math{} may expand to $$
% which is different from $ $ insofar as it starts a displaymath environment 
\long\def\nomath#1{\relax\ifmmode\mbox{#1}\else{#1}\fi}
\newcommand\nlbmath[1]{\nolinebreak\math{#1}}
\newcommand\maths[2]{\math{#1#2}}
\newcommand\nlbmaths[2]{\nolinebreak\math{#1#2}}
%The fol. defines \mathcommand to work like \newcommand with the exception of 
%switching to math-mode iff the command is not called in math-mode.
%\remathcommand is like \renewcommand.

\catcode`\@=11

\long\def\@reargdefmath#1[#2]#3{\@reargdef#1[#2]{\math{#3}}}

\long\def\@argdefmath#1[#2]#3{\@ifdefinable #1{\@reargdefmath#1[#2]{#3}}}

\def\mathcommand#1{\@ifnextchar [{\@argdefmath#1}{\@argdefmath#1[0]}}

\def\remathcommand#1{\edef\@tempa{\expandafter\@cdr\string
  #1\@nil}\@ifundefined{\@tempa}{\@latexerr{\string#1\space undefined}\@ehc
    }{}\@ifnextchar [{\@reargdefmath#1}{\@reargdefmath#1[0]}}

\catcode`\@=12

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mathapplycommand      
#1#2{\mathcommand{#1}[1]{{#2}({##1})}}
\def\mathdoubleapplycommand
#1#2{\mathcommand{#1}[2]{{#2}({##1},{##2})}}
\def\mathtripleapplycommand
#1#2{\mathcommand{#1}[3]{{#2}({##1},{##2},{##3})}}
%example: \mathapplycommand\foo{\rm rubbish}
%         \foo{x} 
%produces:
%         rubbish(x)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\mathoverline=\overline
\remathcommand\overline[1]{\mathoverline{#1}}
% This makes \overline more intelligent, namely switching into math-mode
% if use in text-mode

\newcommand\mycomment[1]{{\iffalse{#1}\fi}}
% The argument of \comment is completely ignored

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Typesetting basics (lengths, struts) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \setlength{\parindent}{2.0em}
\newlength{\disp}
\setlength{\disp}{\textwidth}
\addtolength{\disp}{-2.0\parindent}

\newlength{\textwidthminustwomm}
\setlength{\textwidthminustwomm}{\textwidth}
\addtolength{\textwidthminustwomm}{-0.2cm}

\newlength{\textwidthminushalfcm}
\setlength{\textwidthminushalfcm}{\textwidth}
\addtolength{\textwidthminushalfcm}{-0.5cm}

\newlength{\textwidthminusonecm}
\setlength{\textwidthminusonecm}{\textwidth}
\addtolength{\textwidthminusonecm}{-1.0cm}

\newlength{\textwidthminustwocm}
\setlength{\textwidthminustwocm}{\textwidth}
\addtolength{\textwidthminustwocm}{-2.0cm}

\newlength{\textwidthminusfourcm}
\setlength{\textwidthminusfourcm}{\textwidthminustwocm}
\addtolength{\textwidthminusfourcm}{-2.0cm}

\newlength{\textwidthminussixcm}
\setlength{\textwidthminussixcm}{\textwidth}
\addtolength{\textwidthminussixcm}{-6.0cm}

\newcommand\notop   {\vspace{-1.0\topsep}}
\newcommand\yestop  {\vspace{\topsep}}
\newcommand\halftop {\vspace{0.5\topsep}}
\newcommand\eighthtop{\vspace{0.125\topsep}}
\newcommand\ohyestop{\vspace*{\topsep}}
\newcommand\noitem  {\vspace{-1.0\itemsep}}
\newcommand\yesitem {\vspace{\itemsep}}

\newcommand\schweinerei{
\topsep 4pt plus 1pt minus 2pt
\partopsep 2pt plus 1pt minus 1pt
\renewcommand{\baselinestretch}{0.96}
\hfuzz=4pt}



\newcommand\bigmath[1]{\ \math{#1}\ }
\newcommand\bigmaths[2]{\ \math{#1}#2\ }
\newcommand\mathnlb[2]{\mbox{\math{#1}#2}}
\newcommand\bigmathnlb[2]{\ \mathnlb{#1}{#2}\ }
\newcommand\nlmath{$\hfill\mbox{}\\\mbox{}\hfill$}
\newcommand\nlnomath{\hfill\mbox{}\\\mbox{}\hfill}

%Dont include spaces for pretty print here
\newcommand\linemath[1]{\mbox{}\hfill$#1$\hfill\mbox{}\\}  
\newcommand\linemaths[2]{\mbox{}\hfill$#1$#2\hfill\mbox{}\\}  
\newcommand\linenomath[1]{\mbox{}\hfill{#1}\hfill\mbox{}\\}  
%Dont include spaces for pretty print here
\newcommand\LINEmath[1]{\mbox{}\hfill$#1$\hfill\mbox{}}
\newcommand\LINEmaths[2]{\mbox{}\hfill$#1$#2\hfill\mbox{}}
\newcommand\LINEnomath[1]{\mbox{}\hfill{#1}\hfill\mbox{}}
%Dont include spaces for pretty print here

\newcommand\mysection
[1]{\noindent{\Large\bf#1}\addcontentsline{toc}{section}{#1}}
\newcommand\mysubsection
[1]{\noindent{\Large\bf#1}\addcontentsline{toc}{subsection}{#1}}
\newcommand\mysubsubsection
[1]{\noindent{\bf#1}\addcontentsline{toc}{subsubsection}{#1}}

\newcommand\knuthquotation[2]
{{\footnotesize\begin{flushright}{\sl#1\par}{\noindent\sc--- #2}\end
{flushright}}}

% The fol. \par\noindent\initial{A} writes an initial letter A 
% Note that it was designed to have the bottom line exactly on
% the bottom line of the line it starts. So it works well with
%   \initial{\underline{\underline{\underline{\underline{First case:}}}}}
%   In the first case we have the following...
% The two texts "first case" share their bottom. The underline extends
% below it.
% If you do not want your intials to get the bottom line
% from the bottom line of the first but of the second line
% you must design another macro or use \initial{\raisebox{-3.5ex}{...}}

\newbox\yinibox
\def\initial#1{\par
\noindent
\setbox\yinibox\hbox{#1}%
\setbox\yinibox\vbox to \ht\yinibox{\offinterlineskip\hbox{{#1}~~}\vss}%
\leavevmode
\hangindent=\wd\yinibox
\hangafter=-2
\hbox to0pt{\hskip-\hangindent\box\yinibox\hfill}\ignorespaces}
   
%%% Parentheses: %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mathcommand\inparentheses[1]{\left(\begin{array}[c]{l}#1\end{array}\right)}
\mathcommand\inbracketstight
[1]{\left[\begin{array}[c]{@{}l@{}}#1\end{array}\right]}
\mathcommand\inbrackets[1]{\left[\begin{array}[c]{l}#1\end{array}\right]}
\mathcommand\inbraces[1]{\left\{\begin{array}[c]{l}#1\end{array}\right\}}
\mathcommand\inbracestight
[1]{\left\{\begin{array}[c]{@{}l@{}}#1\end{array}\right\}}
\mathcommand\inparenthesestight
[1]{\left (\begin{array}[c]{@{}l@{}}#1\end{array}\right )}
\mathcommand\inparenthesesinline[1]{(\ #1\ )}
\mathcommand\inpit[1]{(#1)}
\mathcommand\inbracesit[1]{\{#1\}}
\mathcommand\inparenthesesinlinetight[1]{\inpit{#1}}
\newcommand\mathinparenthesesinlinetight[1]{(#1)}%allows line breaking
\mathcommand\noparenthesesoplist[1]
{{\begin{array}{r l}\relax&#1\\\end{array}}}
\mathcommand\noparenthesesoplisttight[1]
{{\begin{array}{@{}r l@{}}\relax&#1\\\end{array}}}
\mathcommand\noparenthesesoplisttop[1]
{{\begin{array}[t]{r l}\relax&#1\\\end{array}}}
\mathcommand\noparenthesesoplisttoptight[1]
{{\begin{array}[t]{@{}r l@{}}\relax&#1\\\end{array}}}
\mathcommand\inparenthesesoplist[1]
{{\left(\noparenthesesoplist{#1}\right)}}
\mathcommand\inparenthesesoplisttight[1]
{{\left(\noparenthesesoplisttight{#1}\right)}}
\mathcommand\inbracesoplist[1]
{{\left\{\noparenthesesoplist{#1}\right\}}}
\mathcommand\inbracketsoplist[1]
{{\left[\noparenthesesoplist{#1}\right]}}
\newcommand\oplistund        {\\\tightund        &}
\newcommand\oplistoder       {\\\tightoder       &}
\newcommand\oplistcup        {\\\tightcup        &}
\newcommand\oplistuplus      {\\\tightuplus      &}
\newcommand\oplistequivalent {\\\tightequivalent &}
\newcommand\oplistimplies    {\\\tightimplies    &}
\newcommand\oplistcirc       {\\\tightcirc       &}
\newcommand\oplistantiimplies{\\\tightantiimplies&}
\newcommand\oplistnl         {\\                 &}
\newcommand\oplistplus       {\\\tight+          &}
\mathcommand\inparenthesesimplies[2]{{\left(\begin{array}{l l}
\multicolumn{2}{l}{#1}\\\tightimplies&#2\\\end{array}\right)}}
\newcommand\inparenthesesimpliestoplevel[3]
{\math{#1\left(\begin{array}{l}\majorheadroom\footroom#2
 \\\end{array}\right.}\\\getittotheright{\math{
 \left.\begin{array}{l l}\tightimplies&\majorheadroom\footroom#3
 \\\end{array}\right)}}} 

\newcommand\opta{{\rm[}}
\newcommand\opte{{\rm]}}
\newcommand\opt[1]{\opta#1\/\opte}
\newcommand\optit[1]{{\it[#1]}}
\mathcommand\displayopt
[1]{\left[\begin{array}[t]{@{\,}c@{\,}}#1\end{array}\right]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MATH NOTATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\stopq{\math{.}\penalty-1\relax\,\,} %\penalty-10 is too low
\mathcommand\hastype[2]{{#1}:\,{#2}}
\mathcommand\tighthastype[2]{{#1}\tight:{#2}}
\mathcommand\prettytighthastype[2]{{#1}\,\tight:\:{#2}}
\mathcommand\typed[3]{#1\hastype{#2}{#3}\stopq}
\mathcommand\comma{,\ \ }
\mathcommand\setwithstart{\{\ }
\newcommand\setwithmark{~\math|\penalty-9\relax\,\ } 
%\penalty-10 is too low, \penalty-1 is too high
\mathcommand\setwithmarkq[1] {\ |_{#1}\ }
\mathcommand\setwithstop     {\ \}}
\newcommand\setwith
[2]{\math{\setwithstart#1}\setwithmark\math{#2\setwithstop}}
%should not be mathcommand for enabling \penalty-1
\mathcommand\displaysetwith
[2]{{\left\{\begin{array}{@{\ \ }l@{\ \ }|@{\ \ }l@{\ \ }}#1&#2\\\end
{array}\right\}}}
\mathcommand\displayset
[1]{{\left\{\begin{array}{@{\ \ }l@{\ \ }}#1\\\end{array}\right\}}}

\newcommand\tight[1]{\math{#1}}
\newcommand\tightsubseteq   {\tight\subseteq  }
\newcommand\tightnotsubseteq{\tight\nsubseteq }
\newcommand\tightsuperseteq {\tight\superseteq}
\newcommand\tightsetminus   {\tight\setminus  }
\newcommand\tightplus       {\tight+          }
\newcommand\tighttimes      {\tight\times     }
\newcommand\tightcap        {\tight\cap       }
\newcommand\tightcup        {\tight\cup       }
\newcommand\tightuplus      {\tight\uplus     }
\newcommand\tightcirc       {\tight\circ      }
\newcommand\tightin         {\tight{\,\in\,}  }
\newcommand\tightnotin      {\tight{\,\not\in\,}  }
\newcommand\tightni         {\tight{\,\ni\,}  }
\newcommand\tightnotni      {\tight{\,\not\ni\,}  }
\newcommand\tightequal      {\tight{\,=\,}\penalty-1\relax}
\newcommand\tightnotequal   {\tight{\,\not=\,}}
\newcommand\tightpreceq     {\tight{\,\preceq\,}}
\newcommand\tightprec       {\tight{\,\prec\,}}
\newcommand\tightnotprec    {\tight{\,\nprec\,}}
\newcommand\tightsucceq     {\tight{\,\succeq\,}}
\newcommand\tightsucc       {\tight{\,\succ\,}}
\newcommand\tightgtr        {\tight{\,>\,}}
\newcommand\tightless       {\tight{\,<\,}}
\newcommand\tightleq        {\tight{\,\leq\,}}
\newcommand\tightgeq        {\tight{\,\geq\,}}

\newcommand\boldequal  {\tight=}
\newcommand\boldunequal{\tight{\not=}}
\newcommand\boldless   {\tight<}
\newcommand\boldnotless{\tight{\not<}}
\newcommand\boldimplies{\tight\tightimplies}
\newcommand\Defnombox{{\rm Def}}
\newcommand\Def{\mbox{\Defnombox}}
\mathcommand\DEF{\Defnombox\:}

%\mathcommand\tightimplies{\rightarrow}    
%\mathcommand\tightantiimplies{\leftarrow}
%\mathcommand\tightequivalent{\leftrightarrow}
\mathcommand\tightimplies{\Rightarrow}
\mathcommand\tightantiimplies{\Leftarrow}
\mathcommand\tightequivalent {\Leftrightarrow}
% The one-line arrow for implication is preferable for the following reasons:
% (1) Hilbert & Bernays uses this symbol.
% (2) In intuitionistic logic, (A->B) can be seen as
%     The type of functions that transform a proof of A
%     to a proof of B, and the implication is valid,
%     if such a function exists.
% The two-line arrow is preferable for the following reason:
% (A) It is more readable in formulas with type declarations and 
%     with \mapsto as a symbol for substitution. Note that the replacement
%     of "x\mapsto y" with "y/x" has two problems again:
%     (a) This would cost me a week to replace it in all contexts.
%     (b) Readability is destroyed by the replacement, because some idiots
%         use "x/y" instead of "y/x".   
% (B) The equivalence looks more like "=" which it actually is.
\mathcommand\tightund        {\wedge}
\mathcommand\tightoder       {\vee}
\mathcommand\tightshefferstroke
% {|}
%Peckhaus: Sheffer stroke sollte größer und fetter sein, etwa mit dem TeX-Befehl \mid (oder verwenden sie ihn schon?).
{\mid}
\mathcommand\tightuparrow{\uparrow}
\def       \implies      {\ \tightimplies      \penalty-2\relax\ }
\newcommand\und          {\ \tightund          \penalty-2\relax\ }
\newcommand\oder         {\ \tightoder         \penalty-2\relax\ }
\newcommand\antiimplies  {\ \tightantiimplies  \penalty-2\relax\ }
\newcommand\equivalent   {\ \tightequivalent   \penalty-2\relax\ }
\newcommand\shefferstroke{\ \tightshefferstroke\penalty-2\relax\ }

\newcommand \id          {{\rm id}}
\mathcommand\allall      {\mathcal{V}}
\mathcommand\allsets     {\POWER\allall}
\mathcommand\allfinitesets{\FINITE\allall}
\mathcommand\urelements  {\mathcal{U}}
\mathcommand\algebra     {\mathcal{A}}
\mathcommand\balgebra    {\mathcal{B}}
\mathcommand\calgebra    {\mathcal{C}}
\mathcommand\dalgebra    {\mathcal{D}}
\mathcommand\ialgebra    {\mathcal{I}}
\mathcommand\salgebra    {\mathcal{S}}
\mathcommand\walgebra    {\mathcal{W}}
\mathcommand\ralgebra    {\mathcal{R}}
\mathcommand\algebraprime{\mathcal{A}'}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathapplycommand\FLD        {\rm field}
\mathapplycommand\DOM        {\rm dom}
\mathapplycommand\RAN        {\rm ran}
\mathapplycommand\kernel     {\rm ker}
% \mathapplycommand\FINITE     {\mbox{\fraknomath P}_\N}%for \frak from german
% \mathapplycommand\POWER      {\mbox{\fraknomath P}}
% \mathapplycommand\posfinPOWER{\mbox{\fraknomath P}_\posN\!}
\mathapplycommand\FINITE     {{\mathfrak P}_{\scriptscriptstyle\N}}%for \frak from amssymb
\mathcommand\POWERSYM        {{\mathfrak P}}
\mathapplycommand\POWER      {\POWERSYM}
\mathapplycommand\posfinPOWER{\POWERSYM_{\scriptscriptstyle\posN\!}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\CARD[1]         {\,|{#1}|\,}
\mathcommand\FLOOR[1]        {\ \lfloor#1\rfloor\ }
\mathcommand\CEIL[1]         {\ \lceil#1\rceil\ }
\mathcommand\reverserelation[1]{{#1}^{-1}}
%\mathcommand\restrictedto[1]{|_{#1}}
\mathcommand\domres[2]{{_{#2}\!\tight\upharpoonleft#1}}
\mathcommand\ranres[2]{{#1\tight\upharpoonright\!_{#2}}}
\mathcommand\funarg[1]{(#1)}
\mathcommand\app[2]{#1(#2)}
\mathcommand\displayapp[2]{#1\inparentheses{#2}}
\mathcommand\displayapptight[2]{#1\inparenthesestight{#2}}
\mathcommand\apptotuple[2]{#1#2}
\mathcommand\relapp[2]{\langle#2\rangle#1}
\mathcommand\displayrelapp
[2]{\left\langle\begin{array}{@{}l@{}}#2\end{array}\right\rangle\!#1}
\mathcommand\relappsin[2]{\relapp{#1}{\!\{#2\}\!}}
\mathcommand\revrelapp[2]{#1\langle#2\rangle}
\mathcommand\displayrevrelapp
[2]{#1\!\left\langle\begin{array}{@{}l@{}}#2\end{array}\right\rangle}
\mathcommand\revrelappsin[2]{\revrelapp{#1}{\!\{#2\}\!}}
\mathcommand\displayrevrelappsin[2]{\displayrevrelapp{#1}{\!\left\{#2\right\}\!}}
\mathcommand\pair[2]{(#1,#2)}
\mathcommand\displaypair[2]{\inparentheses{#1,\ \ #2}}
\mathcommand\displaypairtight[2]{\inparenthesestight{#1,\ #2}}
\mathcommand\trip[3]{(#1,#2,#3)}
\mathcommand\displaytrip[3]{\inparentheses{#1,\ \ #2,\ \ #3}}
\mathcommand\displaytriptight[3]{\inparenthesestight{#1,\ #2,\ #3}}
\mathcommand\superdisplaytrip[3]{\left(\begin
{array}{l}#1,\\#2,\\#3,\\\end{array}\right)}
\mathcommand\quar[4]{(#1,#2,#3,#4)}
\mathcommand\displayquar[4]{\inparentheses{#1,\ \ #2,\ \ #3,\ \ #4}}
\mathcommand\displayquartight[4]{\inparenthesestight{#1,\ #2,\ #3,\ #4}}
\mathcommand\superdisplayquar[4]{\left(\begin
{array}{l}#1,\\#2,\\#3,\\#4\\\end{array}\right)}
\mathcommand\superdisplayquartight[4]{\left(\begin
{array}{@{}l@{}}#1,\\#2,\\#3,\\#4\\\end{array}\right)}
\mathcommand\quin[5]{(#1,#2,#3,#4,#5)}
\mathcommand\displayquin[5]{\inparentheses{#1,\ \ #2,\ \ #3,\ \ #4,\ \ #5}}
\mathcommand\displayquintight[5]{\inparenthesestight{#1,\ #2,\ #3,\ #4,\ #5}}
\mathcommand\sext[6]{(#1,#2,#3,#4,#5,#6)}
\mathcommand\sept[7]{(#1,#2,#3,#4,#5,#6,#7)}
\mathcommand\displaysept[7]
                 {\inparentheses{#1,\ \ #2,\ \ #3,\ \ #4,\ \ #5,\ \ #6,\ \ #7}}
\mathcommand\displaysepttight[7]
                        {\inparenthesestight{#1,\ #2,\ #3,\ #4,\ #5,\ #6,\ #7}}
\mathcommand\oct[8]{(#1,#2,#3,#4,#5,#6,#7,#8)}
\mathcommand\displayocttight[8]
                  {\inparenthesestight{#1,\ #2,\ #3,\ #4,\ #5,\ #6,\ #7,\ #8}}
\mathcommand\ninetuple[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9)}
\newcommand\tentuple[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9,\singletonrest}
\newcommand\singletonrest[1]{#1)}
\newcommand\elev[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9,\pairrest}
\newcommand\pairrest[2]{#1,#2)}
\mathcommand\setwithq[3]     {\setwithstart#2\setwithmarkq{#1}#3\setwithstop}
\mathcommand\setofwords[1]{#1^{\textstyle\ast}}
\mathcommand\setofwordsscriptstyle[1]{#1^{\ast}}
\mathcommand\setofnonemptywords[1]{#1^+}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\FUNSET   [2]{{#1}\rightarrow{#2}}
\mathcommand\PARFUNSET[2]{{#1}\leadsto   {#2}}
\mathcommand\FUNDEF   [3]{\hastype{#1}{\FUNSET   {#2}{#3}}}
\mathcommand\PARFUNDEF[3]{\hastype{#1}{\PARFUNSET{#2}{#3}}}
%categories
\mathcommand\morphcolon{::}
\mathcommand\morpharrow{\rightarrow}
\mathcommand\morph  [3]{{#1}\morphcolon{#2}\morpharrow{#3}}
\newcommand\Idname{{\rm Id}}
\mathcommand\Id[1]{{\Idname_{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\equiclass[2]{{#1}{[\{{#2}\}]}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\aritysugarsymbol{\rightarrow}
\mathcommand\aritysugar{\ \aritysugarsymbol\ }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\monus{\mathchoice
{\raisebox{-.4ex}{$\dot{\raisebox{.4ex}[0ex]{$-$}}$}}%     display-style
{\raisebox{-.4ex}{$\dot{\raisebox{.4ex}[0ex]{$-$}}$}}%     text-style
{\raisebox{-.3ex}{$\scriptstyle\dot{\raisebox{.3ex}[0ex]
{$\scriptstyle-$}}$}}                                %     scriptstyle
{\raisebox{-.2ex}{$\scriptscriptstyle\dot{\raisebox{.2ex}[0ex]
{$\scriptscriptstyle-$}}$}}                          %scriptscriptstyle
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mathcommand\yields{\;\vdash\;}
\mathcommand\antiyields{\;\dashv\;}
\mathcommand\tightyields{\vdash}
\mathcommand\tightantiyields{\dashv}
\mathcommand\notyields{\;\nvdash\;}
\mathcommand\refltransyields{\hspace{0.5em}\raisebox{1.3ex}{\math{\scriptstyle
  \ast}}\hspace{-1.0em}\yields}
\mathcommand\transyields
{\hspace{0.5em}\raisebox{1.3ex}{$\scriptscriptstyle%\oplus
+$}\hspace
{-1.0em}\yields\hspace{0.3em}}
\mathcommand\notmodels{\:\not\!\models}

\newcommand\EVALSYM{{\rm eval}}
\mathapplycommand\EVAL{\EVALSYM}
\mathcommand\formerlycalledepsilon{\ident e}
\mathcommand\V{{\rm V}}
\mathcommand\X{{\rm X}}
\newcommand\nottight{\bigmath}
\mathcommand\refltransclosureinline[1]{{#1}^\ast}
\mathcommand\VARSYM {\mathcal{V}}
\mathapplycommand\VAR{\VARSYM}
\mathcommand\VARnoparentheses[1]{\VARSYM #1}
\mathcommand\VARsingleindex[1]{\VARSYM\!_{{#1}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ZAHLENMENGEN %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \N        Set of natural numbers
% \posN     Set of positive natural numbers
% \ordclass Proper class of ordinal numbers
% \ZZ       Set of integers
% \Q        Set of rationals
% \RE       Set of real numbers
% \posRE    Set of positive real numbers
% \nonnegRE Set of non-negative real numbers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \mathcommand\N{{\rm
% %\rm must be out here because on rare occursions does not work
% %infront of the I\hskip....
% %\ifmmode%  Sind wir im Mathemodus ?
% \mathchoice{{I\hskip -2pt   N}}% display-style
%            {{I\hskip -2pt   N}}% text-style
%            {{I\hskip -1.5pt N}}% scriptstyle
%            {{I\hskip -1pt   N}}% scriptscriptstyle
% %\else\math{\rm I\hskip-2pt N}\fi
% }}
% \newcommand\ZZ{{\rm\ifmmode\mathchoice{{Z\hskip -4pt Z}}{{Z\hskip -4pt Z}}
% {{Z\hskip -3pt Z}}{{Z\hskip -3pt Z}}\else\mbox{\tenrm Z\hskip-4pt Z}\fi}}
\mathcommand\N{{\bf N}}
\mathcommand\posN{\N_{\:\!\!\mbox{\sixsf+}}}
\mathcommand\ZZ{{\bf Z}}
\mathcommand\Q{{\bf Q}}
\mathcommand\ordclass{\mathcal{O}}
%\newcommand\RE{{\rm\ifmmode\mathchoice{{I\hskip -2pt R}}{{I\hskip -2pt R}}
%{{I\hskip -1.5pt R}}{{I\hskip -1pt R}}\else{\tenrm I\hskip-2pt R}\fi}}
\mathcommand\RE{{\bf R}}
\mathcommand\posRE{\RE_{\scriptscriptstyle +}}
\mathcommand\nonnegRE{\RE_{\scriptscriptstyle\succeq0}}

\mathcommand\Qzero{{\cal Q}_0}
\newcommand\squaredot{\,\rule{0.4ex}{0.4ex}\,}

%Transitive closures
\mathcommand\transclosure[1]{\stackrel{\scriptscriptstyle+}{#1}}
\mathcommand\transclosureinline[1]{{#1}^{\scriptscriptstyle+}}

%_____________________________________________________________________________
%Signatures
\mathcommand\sigarity{\alpha}
\newcommand\sig{{\rm sig}}
\mathcommand\sigsorts  {{\mathbb S}}
\mathcommand\sigfunsym {{\mathbb F}}
\mathcommand\consfunsym{{\mathbb C}\,} 
% \, cures strange dvips bugg
\mathcommand\deffunsym {{\mathbb N}}
\mathcommand\Ax{\mathcal{AX}}

%from header.tex
%_____________________________________________________________________________
%Reduction relation

%\red...
%\notred
%\redpara
%\revpara
%\simpara
%\unired
\mathcommand\unired{\Longrightarrow}
\mathcommand\redsimple{\longrightarrow}
\mathcommand\redindex[1]{\redsimple_{_{\!#1}}}
\mathcommand\notredindex[1]{\,\,\,\not\!\!\!\!\redsimple_{_{\!#1}}}
\newcommand\redsub             {\redindex{\R ,\X        }}
\newcommand\redsubprime        {\redindex{\R',\X'       }}
\newcommand\redshortsub        {\redindex{\R ,\V        }}
\newcommand\redshortsubprime   {\redindex{\R',\V'       }}
\newcommand\redsubY            {\redindex{\R ,\Y        }}
\newcommand\redsubemptyset     {\redindex{\R ,\emptyset }}
\newcommand\redsubprimeemptyset{\redindex{\R',\emptyset }}
\newcommand\redsubVsig         {\smallfootroom\redindex{\R ,\Vsig     }}
\newcommand\redsubVsigprime    {\smallfootroom\redindex{\R',\Vsigprime}}
\mathcommand\redindexn[2]{\stackrel{#1}\redsimple_{_{\!#2}}}
\mathcommand\redparaindex[1]{\redpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\revparaindex[1]{\revpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\simparaindex[1]{\simpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\uniredindex[1]{\unired_{\hskip-1.5pt\scriptscriptstyle#1}}

%\antired...
%\notantired..
%\antiredpara...
%\antirevpara...
%\antiunired...
\mathcommand\antiunired{\Longleftarrow}
\mathcommand\antired{\longleftarrow}
\mathcommand\antiuniredindex[1]{\antiunired_{_{\!#1}}}
\mathcommand\antiredindex[1]{\antired_{_{\!#1}}}
\mathcommand\notantiredindex[1]{\,\,\,\not\!\!\!\!\antired_{_{\!#1}}}
\newcommand\antiredsub          {\antiredindex{\R ,\X }}
\newcommand\antiredshortsub     {\antiredindex{\R ,\V }}
\newcommand\antiredshortsubprime{\antiredindex{\R',\V'}}
\newcommand\antiredsubVsig      {\smallfootroom\antiredindex{\R',\Vsig}}
\mathcommand\antiredindexn[2]{\stackrel{#1}\antired_{_{\!#2}}}
\mathcommand\antiredparaindex
[1]{\antiredpara_{\hskip-1.25pt\scriptscriptstyle#1}}
\mathcommand\antirevparaindex[1]
{\antirevpara_{\hskip-1.25pt\scriptscriptstyle#1}}

%\sym...
\mathcommand\sym{\longleftrightarrow}
\mathcommand\symindex[1]{\sym_{_{\!#1}}}
\mathcommand\symindexn[2]{\stackrel{#1}{\sym_{_{\!#2}}}}
\newcommand\symsub     {\symindex{\R,\X}}
\newcommand\symshortsub{\symindex{\R,\V}}
\newcommand\symsubVsig {\smallfootroom\symindex{\R,\Vsig}}

%Reflexive transitive closures
%Congruences
%\congru...
%\footnotecongru...
%\notcongru...
\mathcommand\refltransclosure[1]{\stackrel{\scriptstyle\ast}{#1}}
%{\mathop{#1}^{\scriptstyle\ast}}
\mathcommand\congru{\refltransclosure\sym}
\mathcommand\congruindex[1]{\congru_{_{\!#1}}}
\newcommand\congrusub             {\congruindex{\R ,\X            }}
\newcommand\congrushortsub        {\congruindex{\R ,\V            }}
\newcommand\congrusubVsig         {\smallfootroom\congruindex{\R ,\Vsig     }}
\newcommand\congrusubVsigprime    {\smallfootroom\congruindex{\R',\Vsigprime}}
\newcommand\congrusubemptyset     {\congruindex{\R ,\emptyset     }}
\newcommand\congrusubprimeemptyset{\congruindex{\R',\emptyset     }}
\mathcommand\footnotecongru%{\stackrel\footnoteoast\sym}
{\congru}
\mathcommand\footnotecongruindex[1]{\footnotecongru_{_{#1}}}
\mathcommand\notcongru{\hspace{0.6em}\not\hspace{-0.85em}\refltransclosure\sym}
\mathcommand\notcongruindex[1]{\notcongru_{_{\!#1}}}
\newcommand\notcongrusub        {\notcongruindex{\R,\X       }}
\newcommand\notcongrusubemptyset{\notcongruindex{\R,\emptyset}}

%Transitive closures
%\trans...
%\antitrans...
\mathcommand\trans{\transclosure\redsimple}
\mathcommand\transindex[1]{\trans_{_{\!#1}}}
\newcommand \transsub        {\transindex{\R,\X}}
\newcommand \transshortsub   {\transindex{\R,\V}}
\newcommand \transsubVsig    {\smallfootroom\transindex{\R,\Vsig}}
\newcommand \transsubemptyset{\transindex{\R,\emptyset}}
\mathcommand\antitrans{\transclosure\antired}
\mathcommand\antitransindex[1]{\antitrans_{_{\!#1}}}
\newcommand \antitranssub     {\antitransindex{\R,\X}}
\newcommand \antitransshortsub{\antitransindex{\R,\V}}
\newcommand \antitranssubVsig {\smallfootroom\antitransindex{\R,\Vsig}}

%Reflexive and transitive closures
%\refltrans...
%\footnoterefltrans...
%\notrefltrans...
%\antirefltrans...
%\footnoteantirefltrans...
\mathcommand\refltrans{\refltransclosure\redsimple}
\mathcommand\refltransindex[1]{\refltrans_{_{\!#1}}}
\newcommand \refltranssub          {\refltransindex{\R ,\X }}
\newcommand \refltranssubemptyset  {\refltransindex{\R ,\emptyset}}
\newcommand \refltranssubprime     {\refltransindex{\R',\X'}}
\newcommand \refltransshortsub     {\refltransindex{\R ,\V }}
\newcommand \refltransshortsubprime{\refltransindex{\R',\V'}}
\newcommand \refltranssubVsig      {\smallfootroom\refltransindex{\R ,\Vsig}}
\mathcommand\footnoterefltrans%{\stackrel\footnoteoast\redsimple}
{\refltrans}
\mathcommand\footnoterefltransindex[1]{\footnoterefltrans_{_{#1}}}
\newcommand \footnoterefltranssub     {\footnoterefltransindex{\R,\X}}
\newcommand \footnoterefltransshortsub{\footnoterefltransindex{\R,\V}}
\mathcommand\notrefltrans
            {\hspace{0.6em}\not\hspace{-0.85em}\refltransclosure\redsimple}
\mathcommand\antirefltrans{\refltransclosure\antired}
\mathcommand\antirefltransindex[1]{\antirefltrans_{_{\!#1}}}
\newcommand \antirefltranssub          {\antirefltransindex{\R ,\X }}
\newcommand \antirefltransshortsub     {\antirefltransindex{\R ,\V }} 
\newcommand \antirefltransshortsubprime{\antirefltransindex{\R',\V'}} 
\newcommand \antirefltranssubVsig      {\antirefltransindex{\R',\V'}} 
\mathcommand\footnoteantirefltrans%{\stackrel\footnoteoast\antired}
{\antirefltrans}
\mathcommand\footnoteantirefltransindex[1]{\footnoteantirefltrans_{_{#1}}}
\newcommand \footnoteantirefltranssub     {\footnoteantirefltransindex{\R,\X}}
\newcommand \footnoteantirefltransshortsub{\footnoteantirefltransindex{\R,\V}}

%joinability
\mathcommand\downarrowindex[1]{\downarrow_{_{#1}}}
\newcommand \downarrowsub        {\downarrowindex{\R ,\X       }}
\newcommand \downarrowsubemptyset{\downarrowindex{\R ,\emptyset}}
\newcommand \downarrowsubVsig    {\smallfootroom\downarrowindex{\R,\Vsig}}
\newcommand \downarrowsubprimeemptyset{\downarrowindex{\R',\emptyset}}
\mathcommand\notconfluindex[1]{\notconflu_{_{#1}}}
\newcommand \notconflusub        {\notconfluindex{\R,\X       }}
\newcommand \notconflusubemptyset{\notconfluindex{\R,\emptyset}}
\mathcommand\footnotenotconfluindex[1]{\footnotenotconflu_{_{#1}}}
\newcommand \footnotenotconflusub{\footnotenotconfluindex{\R,\X}}

%strong joinability
\mathcommand\downdownarrow        {\downdownarrows}
\mathcommand\downdownarrowindex[1]{\downdownarrow_{_{#1}}}
\newcommand \downdownarrowsub     {\downdownarrowindex{\R ,\X       }}

\mathcommand\reflclosure[1]{\stackrel
%{\raisebox{0.1em}{$\scriptscriptstyle\preceq$}{ 1}}
{\scriptscriptstyle=}
{#1}}
\mathcommand\reflclosureinline[1]{{#1}^{\scriptscriptstyle=}}
\mathcommand\onlyonce
%{{\displaystyle\mathop{\redsimple}^{{\leq}1}}}
{\reflclosure\redsimple}
\mathcommand\antionlyonce{\reflclosure\antired}
\mathcommand\onlyonceindex[1]{\onlyonce_{_{\!#1}}}
\mathcommand\antionlyonceindex[1]{\antionlyonce_{_{\!#1}}}

\mathapplycommand\nf{\rm NF}

\mathcommand\toconditiontermssub     {\twoheadrightarrow_{_{\R,\X}}}
\mathcommand\toconditiontermssubY    {\twoheadrightarrow_{_{\R,\Y}}}
\mathcommand\toconditiontermsshortsub{\twoheadrightarrow_{_{\R,\V}}}

%_____________________________________________________________________________
%Variables notation
\newcommand \U{{\rm U}}
\newcommand \Y{{\rm Y}}
\newcommand \Z{{\rm Z}}
\mathcommand\Xprime{{\rm X}'}
\mathcommand\Yprime{{\rm Y}'}
\mathcommand\Xprimeprime{{\rm X}''}
\newcommand \SIG     {{\rm SIG}}
\mathcommand\CONS    {\mathcal{C}}
\mathcommand\SIGsort     [1]{(\SIG     ,#1)}
\mathcommand\CONSsort    [1]{(\CONS    ,#1)}
\mathcommand\varsigmasort[1]{(\varsigma,#1)}
\mathcommand\SIGsortindex     [1]{_{\SIG ,#1}}
\mathcommand\CONSsortindex    [1]{_{\CONS,#1}}
\mathcommand\DUNNOsortindex   [1]{_{\DUNNO,#1}}
\mathcommand\varsigmasortindex[1]{_{\varsigma,#1}}
\mathcommand\Vsig      {\V \!_{\SIG }}
\mathcommand\Xsig      {\X   _{\SIG }}
\mathcommand\Vcons     {\V \!_{\CONS}}
\mathcommand\Sigmacons {\Sigmaoffont_{\CONS}}
\mathcommand\Xcons     {\X   _{\CONS}}
\mathcommand\Vconsprime{\V'\!_{\CONS}}
\mathcommand\Vsigprime {\V'\!_{\SIG }}
\mathcommand\sigV      {\Vsig\!\uplus\!\Vcons}
\mathcommand\sigVprime {\Vsigprime\!\uplus\!\Vconsprime}
\mathcommand\hiddenVindi     [2]{\V   \!_{{#1},{#2}}}
\mathcommand\hiddenXindi     [2]{\X     _{{#1},{#2}}}
\mathcommand\hiddenVprimeindi[2]{\V'\!\!_{{#1},{#2}}}
\newcommand \Vsigindex     [1]{\hiddenVindi\SIG     {#1}}
\newcommand \Xsigindex     [1]{\hiddenXindi\SIG     {#1}}
\newcommand \Vconsindex    [1]{\hiddenVindi\CONS    {#1}}
\newcommand \Xconsindex    [1]{\hiddenXindi\CONS    {#1}}
\newcommand \Vvarsigmaindex[1]{\hiddenVindi\varsigma{#1}}
\newcommand \Xvarsigmaindex[1]{\hiddenXindi\varsigma{#1}}
\mathapplycommand\VARCONS{\VARsingleindex\CONS}
\mathapplycommand\VARSIG {\VARsingleindex\SIG}
\mathapplycommand\VARord {\VARsingleindex\boldless}

%_____________________________________________________________________________
%Term notation
\mathcommand\vt{\mathcal{ T}}
\mathcommand\gt{\mathcal{GT}}
\mathcommand\hiddenvtindi[2]{\mathcal{ T}\!_{#1,#2}}
\mathcommand\hiddengtindi[2]{\mathcal{GT}\!_{#1,#2}}
\newcommand\vtsigindex     [1]{\hiddenvtindi{\SIG     }{#1}}
\newcommand\vtconsindex    [1]{\hiddenvtindi{\CONS    }{#1}}
\newcommand\vtvarsigmaindex[1]{\hiddenvtindi{\varsigma}{#1}}
\newcommand\gtsigindex     [1]{\hiddengtindi{\SIG     }{#1}}
\newcommand\gtconsindex    [1]{\hiddengtindi{\CONS    }{#1}}
\newcommand\gtvarsigmaindex[1]{\hiddengtindi{\varsigma}{#1}}
\mathapplycommand\hiddentv     {\mathcal{T}}
\mathapplycommand\hiddentg     {\mathcal{GT}}
\mathapplycommand\hiddentvprime{\mathcal{T}'}
%ground term sets
\newcommand\tgcons              {\hiddentg\cons }
\newcommand\tgsig               {\hiddentg\sig  }   
\newcommand\tgdunno             {\hiddentg\dunno}
\newcommand\tgconsprime         {\hiddentg{\cons'}}
\newcommand\tgsigprime          {\hiddentg{\sig' }}
\newcommand\tgunderlinecons     {\hiddentg{\underline{\underline{\cons }}}}
\newcommand\tgunderlineconsprime{\hiddentg{\underline{\underline{\cons'}}}}
%non-ground term sets
% variables from \Vsig or \Vsigprime
\newcommand\tsigV        {\hiddentv{\sig  ,\V}}
\newcommand\tsigVsig     {\hiddentv{\sig  ,\Vsig}}
\newcommand\tsigVsigprime{\hiddentv{\sig' ,\Vsigprime}}
% variables from \Vcons 
\newcommand\tcc{\hiddentv{\cons,\Vcons}}
% variables from \Vcons\cup\Vsig etc.
\newcommand\tss          {\hiddentv{\sig  ,\sigV     }}
\newcommand\tcs          {\hiddentv{\cons ,\sigV     }}
\newcommand\tcsprime     {\hiddentv{\cons',\sigVprime}}
% variables from \X or \X' etc.
\newcommand\tsigX        {\hiddentv{\sig ,\X }}
\newcommand\tconsX       {\hiddentv{\cons,\X }}
\newcommand\tsigXprime   {\hiddentv{\sig',\X'}}
\newcommand\tconsXprime  {\hiddentv{\cons',\X'}}
\newcommand\tconsVconsX  {\hiddentv{\cons,\Xcons}}
% variables from \Y
\newcommand\tsigY        {\hiddentv{\sig ,\Y }}
\newcommand\tconsY       {\hiddentv{\cons,\Y }}
%term algebras
\newcommand\tconsXalt {\app{{\mathcal T}_\CONS}\X}
\newcommand\tconsValt {\app{{\mathcal T}_\CONS}\V}
\newcommand\tX        {\hiddentv\X}
\newcommand\tXprime   {\hiddentv{\X'}}
\newcommand\tV        {\hiddentv\V}
\newcommand\tY        {\hiddentv\Y}
\newcommand\temptyset {\hiddentv\emptyset}
\newcommand\tVsig     {\hiddentv\Vsig}
\newcommand\tVsigprime{\hiddentvprime\Vsigprime}
% \newcommand{\gtc}{\hiddentg{\cons}}
%_____________________________________________________________________________
%substitutions
\mathcommand\SUBSYM{\mathcal{SU\hspace{-.08em}B}}
\mathdoubleapplycommand\SUBST{\SUBSYM}
\newcommand \Xsubst     {\SUBST\V\tX   }
\newcommand \Vsubst     {\SUBST\V\vt   }
\newcommand \Vsigsubst  {\SUBST\V\tVsig}
\newcommand \Gsubst     {\SUBST\V\gt   }
\mathcommand\Isubst     {{\rm CGSUB}(\V ,\cons )}
\mathcommand\Isubstprime{{\rm CGSUB}(\V',\cons')}
\mathcommand\GENSYM     {\mathcal{G\hspace{-.04em}E\hspace{-.09em}N}}
\mathcommand\GSSYM      {{\GENSYM\hspace{-.14em}}\SUBSYM}
\mathdoubleapplycommand\GS{\GSSYM}
\newcommand\VGS{\GS\V\vt}
\newcommand\XGS{\GS\V\tX}
\newcommand\VsigGS{\GS\V\tVsig}
%
\mathcommand\POSSYMBOL{\mathcal{P\hspace{-.08em}O\hspace{-.1em}S}}
\mathcommand\VPOSSYMBOL{\V\hspace{-.04em}\POSSYMBOL}
\mathcommand\FPOSSYMBOL{\sigfunsym\hspace{-.04em}\POSSYMBOL}
\mathapplycommand\TPOS{\POSSYMBOL}
%\mathapplycommand\POS{\POSSYMBOL} \POS is also used by xy. Use \TPOS instead!
\mathapplycommand\VPOS{\VPOSSYMBOL}
\mathapplycommand\FPOS{\FPOSSYMBOL}
%\mathcommand\OCCSYMBOL{\mathcal{O}}
%\mathapplycommand\OCC{\OCCSYMBOL}%obsolete but still in use
\mathcommand\neitherprefixsymbol{\parallel}
\mathcommand\neitherprefix[2]{{#1}\,\neitherprefixsymbol\,{#2}}
\mathcommand\replsuffix   [2]{[\,#1\leftarrow#2\,]}      %use \repl if possible
\mathcommand\replparsuffix[3]{\replsuffix{#1}{#2\ |\ #3}}%use \replpar
\mathcommand\repl         [3]{#1\penalty-1\replsuffix{#2}{#3}}
\mathcommand\replpar      [4]{#1\penalty-1\replparsuffix{#2}{#3}{#4}}
\mathcommand\eqvariablessig[1]{\mbox{\rm Eq}(\sig,{#1})}
\newcommand\eqvsig{\eqvariablessig{\sigV}}
\mathcommand\eqgsig{\mbox{\rm GEq}(\sig)}
\mathcommand\direqv[1]{\mbox{\rm DEq}(#1)}
\newcommand\direqvariablessig[1]{\direqv{\sig,{#1}}}
\newcommand\direqvsig{\direqv{\sig,\sigV}}
\mathapplycommand\MGU{\rm Mgu}
\mathdoubleapplycommand\minmgu{\rm mgu}
\mathdoubleapplycommand\sep{\rm Sep}
\mathdoubleapplycommand\minsep{\rm sep}
\mathapplycommand\depth{\rm depth}
\mathapplycommand\size{\rm size}
\newcommand\monotonic           {\tsigX-mono\-tonic}
\newcommand\Vmonotonic          {\vt-mono\-tonic}
%\newcommand\amonotonic          {an \X-mono\-tonic}
\newcommand\emptysetmonotonic   {\gt-mono\-tonic}
\newcommand\monotonicity        {\tsigX-mono\-toni\-city}
\newcommand\Vmonotonicity       {\vt-mono\-toni\-city}
%\newcommand\Monotonicity        {\X-mono\-toni\-city}
\newcommand\stable              {\X-stable}
\newcommand\Vstable             {\V-stable}
\newcommand\Ystable             {\Y-stable}
\newcommand\emptysetstable      {\mbox{$\emptyset$}-stable}
\newcommand\stability           {\X-stabi\-lity}
\newcommand\Stability           {\X-stabi\-lity}
\newcommand\Vstability          {\V-stabi\-lity}
\newcommand\VStability          {\V-stabi\-lity}
\newcommand\compatible          {\X-compa\-tible}
\newcommand\RXcompatible        {\RX-compa\-tible}
\newcommand\Vcompatible         {\V-compa\-tible}
\newcommand\Ycompatible         {\Y-compa\-tible}
\newcommand\leftrightcompatible {\X-left-right-compa\-tible}
\newcommand\Vleftrightcompatible{\V-left-right-compa\-tible}
\newcommand\dontcarecompatible  {\X-don't-care-compa\-tible}
\newcommand\aleftrightcompatible{an \X-left-right-compa\-tible}
\newcommand\adontcarecompatible {an \X-don't-care-compa\-tible}
\newcommand\compatibility       {\X-compa\-ti\-bility}
\newcommand\dontcarecompatibility{\X-don't-care-compa\-ti\-bility}
\newcommand\Vdontcarecompatible {\V-don't-care-compa\-tible}
\newcommand\Safety              {Safeness}
\newcommand\safety              {safeness}
\newcommand\safe                {safe}
\newcommand\Safe                {Safe}
\newcommand\unsafe              {unsafe}
\newcommand\safely              {safely}
\newcommand\constructorminimal{con\-struc\-tor-mini\-mal}
\newcommand\ConstructorMinimal{Con\-struc\-tor-Mini\-mal}
\newcommand\constructorminimality{con\-struc\-tor-mini\-mal\-ity}
\newcommand\constructorminimum{con\-struc\-tor-mini\-mum}
\newcommand\constructorpreserving{con\-struc\-tor-pre\-serving}
\newcommand\constructorpreservation{con\-struc\-tor-pre\-serva\-tion}
\newcommand\constructorbased{con\-struc\-tor-based}
\newcommand\Constructorbased{Con\-struc\-tor-based}
\newcommand\terminationpair{termi\-na\-tion-pair}
\newcommand\TerminationPair{Termi\-na\-tion-Pair}
\newcommand\inductivesubstitution{constructor ground substitution}
\newcommand\aninductivesubstitution{a constructor ground substitution}
\newcommand\Inductivesubstitution{Constructor ground substitution}
\newcommand\InductiveSubstitution{Constructor Ground Substitution}
\newcommand\inductiveinstance{constructor ground instance}

%Subterm
\newcommand\hiddensubST{_{_{\rm ST}}}
\mathcommand\superterm   {\rhd\hiddensubST}
\mathcommand\notsuperterm{\ntriangleright\hiddensubST}
\mathcommand\subterm     {\lhd\hiddensubST}
\mathcommand\notsubterm  {\ntriangleleft\hiddensubST}
\mathcommand\supertermeq {\trianglerighteq\hiddensubST}
\mathcommand\subtermeq   {\trianglelefteq\hiddensubST}

\mathcommand\sugarregel{l\boldequal r\rulesugar C}
\mathcommand\sugarregelindex[1]{l_{#1}\boldequal r_{#1}\rulesugar C_{#1}}
\mathcommand\sugaruncondregelindex[1]{l_{#1}\boldequal r_{#1}}
\mathcommand\ndrulewithassumption[3]{{{{\scriptstyle\lbrack}#1{\scriptstyle
\rbrack}}\atop\scriptstyle #2}\over #3}

%_____________________________________________________________________________
%Rules
\def\R{{\rm R}}
\mathcommand\RCONS{\R_\CONS}
\mathcommand\Rprime{{\rm R}'}
\mathcommand\RX{\R,\X}
\mathcommand\RCONSX{\RCONS,\X}
\mathcommand\DEFUNSYM{\mathcal{DEFUN}}
\mathapplycommand\DEFUN{\DEFUNSYM}
\newcommand\defsort{{\rm def}}
\mathcommand\ATSYM  {\mathcal{A\hspace{-.02em}T}}
\mathdoubleapplycommand\atomsof{\ATSYM}
\newcommand\atoms      {\atomsof\sig\V}
\newcommand\Xatoms     {\atomsof\sig\X}
\newcommand\Yatoms     {\atomsof\sig\Y}
\newcommand\scatoms    {\atomsof\sig\Vcons}
\mathcommand\GENATSYM  {\GENSYM\hspace{-.18em}\ATSYM}
\mathdoubleapplycommand\genatomsof{\GENATSYM}
\newcommand\genatoms      {\genatomsof\sig\V}
\newcommand\Xgenatoms     {\genatomsof\sig\X}
\newcommand\Ygenatoms     {\genatomsof\sig\Y}
\mathcommand\CONDSYM  {\mathcal{C\hspace{-.1em}O\hspace{-.12em}N\hspace{-.12em}D}}
\mathcommand\LITSYM   {\mathcal{LI\hspace{-.04em}T}}
\mathcommand\CONDLITSYM{\CONDSYM\hspace{-.04em}\LITSYM}
\mathapplycommand\condlitwitharg{\CONDLITSYM}
\newcommand\condlit {\condlitwitharg{\sig,\V}}
\newcommand\Xcondlit{\condlitwitharg{\sig,\X}}
\newcommand\Ycondlit{\condlitwitharg{\sig,\Y}}
\mathdoubleapplycommand\literals{\LITSYM}
\newcommand \lit        {\literals\sig\V}
\newcommand \Xlit       {\literals\sig\X}
\newcommand \Ylit       {\literals\sig\Y}
\mathcommand\GENLITSYM{\GENSYM\hspace{-.08em}\LITSYM}
\mathdoubleapplycommand\genliterals{\GENLITSYM}
\newcommand \genlit        {\genliterals\sig\V}
\newcommand \Xgenlit       {\genliterals\sig\X}
\newcommand \Ygenlit       {\genliterals\sig\Y}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

